Learning Spatial Common Sense with Geometry-Aware Recurrent Networks

We integrate two powerful ideas, geometry and deep visual representation learning, into recurrent network architectures for mobile visual scene understanding. The proposed networks learn to "lift" and integrate 2D visual features over time into latent 3D feature maps of the scene. They are equipped with differentiable geometric operations, such as projection, unprojection, egomotion estimation and stabilization, in order to compute a geometrically-consistent mapping between the world scene and their 3D latent feature state. We train the proposed architectures to predict novel camera views given short frame sequences as input. Their predictions strongly generalize to scenes with a novel number of objects, appearances and configurations; they greatly outperform previous works that do not consider egomotion stabilization or a space-aware latent feature state. We train the proposed architectures to detect and segment objects in 3D using the latent 3D feature map as input--as opposed to per frame features. The resulting object detections persist over time: they continue to exist even when an object gets occluded or leaves the field of view. Our experiments suggest the proposed space-aware latent feature memory and egomotion-stabilized convolutions are essential architectural choices for spatial common sense to emerge in artificial embodied visual agents.

==> experiments_old.tex <==
\section{Experiments}\label{sec:exp}
\begin{figure}[h!]
	\centering
	\includegraphics[width=0.5\textwidth]{figures/viewprediction_small.pdf}
\caption{
	\textbf{View prediction results} for the proposed \slamrnn and the tower model (a version of 2D RNN )  of Eslami et al. \cite{Eslami1204}. Columns from left to right show the three input views,  the ground-truth image from the query viewpoint,  the view predictions for \slamrnn and for the tower baseline. 
		The first two rows are from the  ShapeNet arrangement test set of \cite{activevision}, and the next two rows are from the Shepard-Metzler test set of \cite{Eslami1204}. The last fours rows show generalization to  scenes with four objects from ShapeNet arrangement dataset, while both models were  trained only in scenes with two objects. \slamrnn outperform the baseline by a margin and  \textit{strongly} generalize under varying number of objects. 
	}
	\label{fig:viewprediction}
\end{figure}


%We test  \slamrnn on the tasks of  view prediction and 3D object detection and segmentation. %All experiments concern  static scenes under a moving observer. 
%In all cases, we compare against  models  that do not consider egomotion-stabilized convolutions or a 3D  latent feature state space.  



%Our experiments are carried out in the following simulation datasets:
%i)  scenes we create using synthetic 3D object models from  ShapeNet~\cite{shapenet2015}.  The generated scenes contain  single or multiple objects on a table surface.
%ii)\todo{ricson}
%iii)
%scenes from the SUNCG~\cite{song2016ssc} dataset, sampled around an object of interest. 



%\input{view_pred_fig.tex}
%\input{arith_fig.tex}

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.5\textwidth]{figures/arithmetics_small.pdf}
	\caption{\textbf{Scene arithmetics} from the proposed \slamrnn and the model  of Eslami et al. \cite{Eslami1204} (tower). Each row is a separate "equation". We start with the representation of the  scene in the leftmost column, then subtract (the representation of) the scene in the second column, and add the (representation of the) scene in the third column. We decode the resulting  representations into an image view. The groundtruth is shown in the forth column and is much more visually similar to the prediction of \slamrnn than to the tower baseline.}
	\label{fig:arithmetics}\label{key}
\end{figure}


%Teaching machines spatial common sense is a long desired goal for Artificial Intelligence

  The term ``spatial common sense" is broad and concerns the ability to perceive and understand properties and regularities regarding spatial arrangements and motion that are is shared by (``common to") nearly all people, for example, that fact that objects have 3D shape as opposed to being floating 2D surfaces, the fact that scenes are comprised of objects, the 3D non-intersection principle, the fact that objects do not spontaneously disappear, and many others.  \cite{DBLP:journals/corr/abs-1212-4799}.
%among many  object motion,  object permanence, that fact that objects have 3D shape as opposed to being floating 2D surfaces, the fact that scenes are comprised of objects, the 3D non-intersection principle, and many others. 
The   model we propose in this work targets understanding of \textit{static} scenes,  that is, scenes that do not contain  any independently moving objects, and that are  viewed under a (potentially) moving observer.  Thus, we restrict the term \textit{spatial common sense} to refer to rules and regularities that can be perceived  in static worlds.
Our experiments  aim to answer the following questions:
\begin{enumerate}
    \item Do \slamrnn learn spatial common sense?
    \item Are geometric structural biases necessary for spatial common sense to emerge?
    %\item Does object detection in the 3D latent feature map outperforms view (frame) based detectors?
    %\item Do \slamrnn outperform geometry-unaware alternatives in 3D object detection?
\end{enumerate}

We train and test our models and baselines from recent previous works in the tasks of view prediction and 3D object detection, to answer those questions. 

\subsection{View prediction} 


We consider the following simulation datasets: 
i)  \textit{ShapeNet arrangement}  from ~\cite{activevision} which consist of scenes that have synthetic 3D object models from ShapeNet~\cite{shapenet2015} arranged on a table surface. Objects belong to four object categories, namely, cups, bowls, helmets, cameras. We follow the same train/test split of ShapeNet~\cite{shapenet2015}  so that object instances which appear in train  scenes do not appear in the test  scenes. Each scene contains two objects, and each image is rendered from a viewing sphere which has $3\times18$ possible views with 3 camera elevations $(20^{\circ}, 40^{\circ}, 60^{\circ})$ and 18 azimuths $(0^{\circ}, 20^{\circ}, \dots, 340^{\circ})$. There are 300 different scenes in the training set and 32 scenes
with novel objects in the test set.  
%We train  on scenes that contain  two objects. We test our model and baselines both on scenes that contain two objects, as well as, scenes that contain four objects, to evaluate the strong generalization of our model and baselines. %and also see how models trained on such scenes generalize to scenes containing  four objects. 
%We also have "scene arithmetic" experiments consisting of scenes with variable number of objects in them. 
ii) \textit{Shepard-metzler } from ~\cite{Eslami1204}. These scenes consist of seven colored cubes stuck together in random arrangements. We use the train and test split of ~\cite{Eslami1204}. 
iii) \todo{...}, included in the supplementary material, in order to save space. 

We compare the proposed \slamrnn   against the recent tower architecture of  Eslami et al. \cite{Eslami1204}, a 2D LSTM network  trained under a similar view prediction loss, that has a 2D instead of 3D feature space, and no egomotion-stabilized convolutions. Both models share the same autoregressive decoder. 
For simplicity, we use groundtruth egomotion rather than estimated egomotion in all view prediction experiments for both our model and the tower baseline. 



Test results from our model and baseline on test images in ShapeNet arrangements and Shepard-metzler datasets are shown in Figure \ref{fig:viewprediction}.  Reconstruction errors for the ShapeNet arrangement dataset are shown in Table \ref{tab:viewpredtable}. \slamrnn have a much lower reconstruction test error than the tower baseline. In Figure \ref{fig:viewprediction}, in the first four rows,  the distribution of the test scenes matches the training distribution. Our model  outperforms the baseline in visual quality. 
%,
In Figure \ref{fig:viewprediction}, in the last four rows, the test scene distribution does not match the training one: we test our model and baseline on  \textbf{scenes with four objects, while both models are trained on scenes with exactly two objects. } 
In this case, our model outperforms by a margin the our geometry-unaware baseline of  \cite{Eslami1204}, showing \textit{strong generalization}.  Indeed, the ability for spatial reasoning should not be affected by the number of the objects present in the scene. %Common sense acquisition we argue entails strong generalization: 
%The baseline was not able to generalize effectively to novel objects and configurations. 
The results above suggest that geometry-unaware models may be merely memorizing views with small interpolation capabilities, as opposed to learning to spatially reason. We attribute this to their inability to represent space efficiently in their latent vectors, a problem the proposed architectures correct for.


\paragraph{Scene arithmetics}
The learnt  representations of \slamrnn under view prediction are capable of scene arithmetics, as we show in Figure \ref{fig:arithmetics}.  The ability to add and subtract individual objects from 3D scenes just by adding and subtracting their corresponding latent representations demonstrates what/where disentanglement achieved by our model. Our  3D feature memory learns to store object-specific information in the regions of the  memory which correspond to the  spatial location of the corresponding object in the scene. Therefore, it is relatively straightforward to carry out scene arithmetics with our model.

\paragraph{Implementation details} 
The view prediction results we show in Figure \ref{fig:viewprediction} and in the supplementary material were obtained after training for ~24H on one GPU, for both our model and the baseline. 
 %We would like to note here that both models are trained for approximately the same number of iterations. 
 We are still training the baseline in case we can further improve its reconstruction quality, since the authors of \cite{Eslami1204} mention  they trained their model for a month on \todo{++} GPUs. Although this may improve eventually the quality of the predicted views in case of same train/test distributions, it is unlikely to improve the generalization capability of the tower baseline. We will update the baseline results once the extended training completes.  %More qualitative results are included in the supplementary material. 
 Further details of the model architecture and baseline are included in the supplementary material.  

\begin{table}[htbp!]
\centering
\begin{tabular}{c|cc}
            \multicolumn{1}{l|}{}          &  \multicolumn{1}{l}{Tower} & \multicolumn{1}{l}{GRNNs} \\ \hline
ShapeNet arrangements & $0.109 \pm 0.029$ & ${\bf 0.084} \pm 0.017$ \\
Shepard-Metzler & $0.081 \pm 0.017$ & ${\bf 0.073} \pm 0.014$ \\
\end{tabular}
\caption{\textbf{View prediction  (cross-entropy) loss and the standard deviation} for the ShapeNet arrangement test set of two-object scenes. Our model and baseline were trained on  scenes that also contain two objects with different object instances.}
\label{tab:viewpredtable}
\end{table}



\begin{comment}

\begin{table}[htbp!]
\centering
\begin{tabular}{c|cc}
\multicolumn{1}{l|}{\# views aggregated}          &  \multicolumn{1}{l}{2D-RNNs} & \multicolumn{1}{l}{GRNNs} \\ 
\multicolumn{1}{l|}{ in 
current memory}          &  \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
1& $3.2 / 23.1$ & $8.6/ 17.8$ \\
2& $3.1 / 25.1$ & $5.6/16.8$ \\
3& $3.5 / 18.6$ & $5.6/ 6.6$ \\
\hline
avg &${\bf 3.3}/22.2$ & $6.9/{\bf 13.7}$\\
\end{tabular}
\caption{ Elevation and azimuth angle error for ego-motion prediction.  }
\label{tab:egotable}
\end{table}


\end{comment}





\begin{table}[htbp!]
	\centering
	\begin{tabular}{c|c}
		\multicolumn{1}{l|}{\# views aggregated}          & \multicolumn{1}{l}{GRNNs} \\ 
		\multicolumn{1}{l|}{ in 
			 memory}         & \multicolumn{1}{l}{} \\ \hline
		1 & $8.6/ 17.8$ \\
		2 & $5.6/16.8$ \\
		3& $5.6/ 6.6$ \\
		\hline
		avg & $6.9/13.7$\\
	\end{tabular}
	\caption{ Elevation and azimuth angle error for ego-motion prediction.  }
	\label{tab:egotable}
\end{table}



\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/3Dmaskrcnn.jpg}
     \caption{\textbf{3D object detection}. Blue voxels show ground truth objects. Predicted 3D boxes and their corresponding predicted masks are show in red and green. }    
    
    %\caption{\textbf{3D obejct detection}. Red and blue voxels show ground truth objects. Predicted 3D boxes are  shown in red and green. }
    \label{fig:bbox_visual}
    
\end{figure*}
 

\subsection{3D object detection}

%\subsection{Egomotion estimation}
%Our model at each frame estimates the egomotion of the observer with respect to the 3D feature map,  stabilizes against it, updates the memory tensor and detects objects with a 3D region proposal network. We first describe our egomotion and quantify its error. We then benchmark our object detector against a 2D recurrent network. 

We use the ShapeNet arrangement 3D scenes from \cite{activevision} described in the previous section. 
%: each scene contains two objects, and each image is rendered from a viewing sphere which has $3\times18$ possible views with 3 camera elevations $(20^{\circ}, 40^{\circ}, 60^{\circ})$ and 18 azimuths $(0^{\circ}, 20^{\circ}, \dots, 340^{\circ})$. There are 300 different scenes in the training set and 32 scenes
%with novel objects as test set.  
During training, a sequence of four views is randomly selected 
and the model is trained to predict relative camera motion with respect to the  memory map integrated from the views seen thus far. 
We estimate the elevation of the first camera view, and orient our 3D feature memory to have 
%The 3D feature memory are oriented to have 
$0^{\circ}$ in elevation. This essentially means our memory is parallel to the ground plane. The azimuth of the 3D feature memory is aligned with the azimuth of the 
first view in the input sequence. 



%We set up a baseline model by removing all the 3D operations, e.g., unprojection, rotation, projection. The model takes as input an image, pass it through a encoder-decoder tower with skip connection to obtain a 2D feature tensor. The camera parameters for this view are concatenated as additional channels to the 2D feature tensor and altogether they are passed through another encoder-decoder tower to obtain the 2D feature tensor for memory update. The memory is updated using 2D GRU. The final view is selected based on the inner products between current memory and 2D feature obtained using different views, similar to what we have in the proposed model. 

In Table \ref{tab:egotable}, we show prediction error in terms of elevation and azimuth angles. Our model improves its egomotion estimates with more views aggregated to the memory. 
%The proposed GRNNs on average performs better than 2D-RNNs baseline and is $9$ degree better in relative azimuth prediction. 
Note that since we always rotate the scene to have 0 elevation, it is possible for the network to predict the elevation directly from the query image without looking at other images, while for the azimuth, since it is the relative angles to the first view, it is necessary for the network to take  into account previously 
seen images. 

%Besides, our results show GRNNs are able to improve with more views aggregated to the memory while 2D-RNNs do not have such property.



%We consider the viewing angles available in the dataset \todo{???}. 
%For each scene, 
%We create a simulated environment where the camera is able to move around, by rendering

%We next benchmark our 3D object detector. We use the same ShapeNet arrangement dataset, and train/test split. 

We sample a sequence 
of four views and predict 3D object boxes  at each time step.

 We consider the following baseline model, which we call \textit{2D-RNN}: We remove the unprojection, rotation, and projection \todo{??} from our model. The baseline takes as input an image, feeds it to a 2D encoder-decoder network with skip connection to obtain a 2D feature tensor. The camera parameters for this view are concatenated as additional channels to the 2D feature tensor and altogether they are fed  to another 2D encoder-decoder network to obtain the 2D feature tensor for memory update. The memory is a 2D GRU network.  
We then feed the 2D memory feature tensor to an encoder-decoder
network to get a prediction output and we reshape the channel dimension into $d$ feature vector \todo{?} to form a 4D tensor as prediction.

%The final view is selected based on the inner products between current memory and 2D feature obtained using different views, similar to what we have in the proposed model. 



%We use the same ShapeNet dataset as egomotion estimation where
%each scene contains two objects. Similarly, 

%we draw a sequence 
%for four views and predict at each time step. Since the final predictions 
 %are 3D tensors (one indicating positive anchors and one indicating refinement at each location), for the 2D-RNNs baseline,
 %we first pass the 2D memory feature tensor through an encoder-decoder
 %tower to get and prediction output and we reshape the channel dimension into $d$ feature vector to form a 4D tensor as prediction. 
 

 
 
 Table \ref{tab:maptable} shows that GRNNs are significantly better than
 2D-RNNs in terms of mean average precision (mAP) for object detection.
\todo{We futher show that if extra depth map is available, during unprojection, for each ray cast, we keep only features around the depth value. This further improves our object detection performance.}  We  visualize the 
 predicted 3D bounding boxes from GRNNs with depth in Figure \ref{fig:bbox_visual}.

 
 
 \todo{To show how 2D-RNNs fails,} Figure \ref{fig:bbox_positive} illustrates positive anchor predictions from the two models: while 2D-RNNs are able to predict correct boxes  from the front view, they fail to predict the correct position along the depth channel. Note that our model never uses depth information during training, it learns it implicitly.  
\begin{table}[htbp!]
\centering
\begin{tabular}{c|ccc}
            \multicolumn{1}{l|}{}          &  \multicolumn{1}{l}{2D-RNNs} & \multicolumn{1}{l}{GRNNs} & \multicolumn{1}{l}{GRNNs (with depth)} \\ \hline
$mAP_{0.75}^{bbox}$ & $0.025$ &  $0.145$ & ${\bf 0.348}$\\
$mAP_{0.50}^{bbox}$ & $0.323$ &  $0.917$ & ${\bf 0.977}$\\
$mAP_{0.33}^{bbox}$ & $0.653$ &  $0.981$ & ${\bf 0.991}$\\
\end{tabular}
\caption{ Mean Average Precision (mAP) for 3D object detection on ShapeNet arrangement \cite{activevision} testset.}
\label{tab:maptable}
\end{table}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/bbox_positive_map2_small.pdf}
    \caption{3D binary tensor indicating positive anchor locations is projected onto the front view and bird view. The groundtruth is aligned to the first view in azimuth. The last two columns in the top and bottom images show predictions from 2D-RNNs and GRNNs, respectively. Images from top to bottom is predictions in different time steps.
    GRNNs is able to infer correct locations even under serious occlusion in the first frame  while 2D-RNNs fails to predict along the depth dimension
    for relatively simple scene.}
    \label{fig:bbox_positive}
    
\end{figure}





\todo{
Next, we show mAP for object detection mask in Table \ref{tab:map_mask_table}. For 2D-RNNs baseline, we concatenate 
the extra depth map along with rgb features as input to the network. 
Our results show the proposed geometry-aware RNNs are} significantly better.

\begin{table}[htbp!]
\centering
\begin{tabular}{c|ccc}
            \multicolumn{1}{l|}{}          &  \multicolumn{1}{l}{2D-RNNs}  & \multicolumn{1}{l}{GRNNs} & \multicolumn{1}{l}{GRNNs} \\
            \multicolumn{1}{l|}{}          &  \multicolumn{1}{l}{ w. gt depth} &  \multicolumn{1}{l}{ w. learnt depth} & \multicolumn{1}{l}{ w. gt depth} \\  
            
            \hline
$mAP_{0.75}^{mask}$ & $0.00$ & $0.00$ &${\bf 0.110}$ \\
$mAP_{0.5}^{mask}$ & $0.006$ & $0.066$ &${\bf 0.378}$ \\
$mAP_{0.33}^{mask}$ & $0.104$ & $0.289$ & ${\bf 0.545}$ \\
\end{tabular}
\caption{ Mean Average Precision (mAP) for 3D object detection masks on ShapeNet arrangement \cite{activevision} testset.}
\label{tab:map_mask_table}
\end{table}

Last, we show object detection results using estimated egomotion in Table \ref{tab:map_ego_mask_table}. 
\begin{table}[htbp!]
\centering
\begin{tabular}{c|c||c|c}
            \multicolumn{1}{l|}{bbox mAP}          &  \multicolumn{1}{l||}{GRNNs}  & \multicolumn{1}{l|}{mask mAP} & \multicolumn{1}{l}{GRNNs} \\
            \multicolumn{1}{l|}{}          &  \multicolumn{1}{l||}{ w. gt depth} &  \multicolumn{1}{l|}{} & \multicolumn{1}{l}{ w. gt depth} \\  
            
            \hline
$mAP_{0.75}^{bbox}$ & $0.339$ & $mAP_{0.75}^{mask}$ &$0.049$ \\
$mAP_{0.5}^{bbox}$ & $0.971$ & $mAP_{0.5}^{mask}$ &$0.323$ \\
$mAP_{0.33}^{bbox}$ & $0.995$ & $mAP_{0.33}^{mask}$ & $0.436$ \\
\end{tabular}
\caption{ Mean Average Precision (mAP) for 3D object detection using estimated egomotion.}
\label{tab:map_ego_mask_table}
\end{table}




Please, see our supplementary material for architecture and training details, and much more qualitative results, as well as videos of our predictions. 






\iffalse
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/egomotion.pdf}
    \caption{Ego-motion prediction accuracy of different time steps during training. GRNNs is consistently better than 2D-RNNs and the prediction improves over time while 2D-RNNs does not appear to have such property. }
    \label{fig:ego_motion}
    
\end{figure}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/rpn.pdf}
    \caption{Negative log likelihood loss for anchors prediction and regression loss for bounding box prediction. GRNNs is marginally better than 2D-RNNs in both matrices.   }
    \label{fig:bbox_positive}
    
\end{figure}
\fi








